Events and Controversies: Influences of a Shocking News Event on Information Seeking

It has been suggested that online search and retrieval contributes to the intellectual isolation of users within their preexisting ideologies, where people's prior views are strengthened and alternative viewpoints are infrequently encountered. This so-called "filter bubble" phenomenon has been called out as especially detrimental when it comes to dialog among people on controversial, emotionally charged topics, such as the labeling of genetically modified food, the right to bear arms, the death penalty, and online privacy. We seek to identify and study information-seeking behavior and access to alternative versus reinforcing viewpoints following shocking, emotional, and large-scale news events. We choose for a case study to analyze search and browsing on gun control/rights, a strongly polarizing topic for both citizens and leaders of the United States. We study the period of time preceding and following a mass shooting to understand how its occurrence, follow-on discussions, and debate may have been linked to changes in the patterns of searching and browsing. We employ information-theoretic measures to quantify the diversity of Web domains of interest to users and understand the browsing patterns of users. We use these measures to characterize the influence of news events on these web search and browsing patterns.

==> 023userCategories.tex <==
%\subsection{Categories of users}
\label{sec:categories}

In the following sections, in addition to the total users, we also refer to the ``active'' and ``common'' users, depending on the type of analysis we are doing. 

\paragraph{``Active'' users}
\label{sec:active}
We characterize as {\it active} the users who had at least 3 relevant browsing sessions during December, and visited at least 5 different domains. Among the 221 active users in our dataset, 54 of them visited gun-related websites both before and after the shooting. Our goal is to analyze the browsing behaviors of these users in depth, as there exists enough browsing data for them (they have not just visited 1 or 2 websites), and all the webpages they have visited are labeled based on their stance. 

%The distributions of distinct domains visited by these users, as well as the sessions are given in Figures~\ref{fig:distDomains} and \ref{fig:distSessions} respectively.
%
%\begin{figure}[h!]
%  \centering
%      \includegraphics[width=0.5\textwidth]{FIG/domain_distribution_for_active_users}
%  \caption{Distribution of unique domains visited by the {\it active} users during December.}
%           \label{fig:distDomains}
%\end{figure}
%
%\begin{figure}[h!]
%  \centering
%      \includegraphics[width=0.5\textwidth]{FIG/session_distribution_for_active_users}
%  \caption{Distribution of gun-related sessions for the {\it active} users during December.}
%           \label{fig:distSessions}
%\end{figure}




\paragraph{Common users}

In this paper, we are interested in understanding the effect of external events to the polarization of the users. As it is obvious in Fig.~\ref{fig:temporal}, many new users are observed each day, and especially after the shooting. To understand the polarity shift and remove the effect of new users, in some parts of our study we refer to the group of users that have relevant \nonNews sessions both before and after \SH. We refer to them as common users, and the relevant dataset as \nonNewsCommon(Table~\ref{tab:commonUsers}). As mentioned above, there exist 54 common, active users.

% Table generated by Excel2LaTeX from sheet 'Statistics'
\begin{table}[htbp]
  \centering
  \caption{Statistics for the \nonNewsCommon dataset. The last column holds the number of common users, URLs and domains between the two time periods.}
  \resizebox{\columnwidth}{!}{
    \begin{tabular}{rrrrr}
    \toprule
     & \multicolumn{1}{c}{\textbf{Before \SHshort}} & \multicolumn{1}{c}{\textbf{After \SHshort}} & \multicolumn{1}{c}{\textbf{Total}} & \multicolumn{1}{c}{\textbf{Overlap}} \\
    \midrule
    \textbf{Users} & 846   & 846   & 846   & 846 \\
        \textbf{Sessions} & 2,018 & 3,544 & 5,562 & N/A \\
        \textbf{Unique URLs} & 4,011 & 7,499 & 10,431 & 1,079 \\
        \textbf{Unique Domains} & 82    & 125   & 160   & 47 \\
        \textbf{Total Entries} & 23,844 & 42,314 & 66,158 & N/A \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:commonUsers}%
\end{table}%

%The distributions of distinct domains visited by these users, as well as the sessions are given in Figures~\ref{fig:distDomainsCommon} and \ref{fig:distSessionsCommon} respectively.

%\begin{figure}[h!]
%  \centering
%      \includegraphics[width=0.5\textwidth]{FIG/domain_distribution_for_active_users_COMMON}
%  \caption{Distribution of unique domains visited by the {\it active} users who have gun-control-related activity before and after \SH.}
%           \label{fig:distDomainsCommon}
%\end{figure}

%\begin{figure}[h!]
%  \centering
%      \includegraphics[width=0.5\textwidth]{FIG/session_distribution_for_active_users_COMMON}
%  \caption{Distribution of gun-related sessions for the {\it active} users who have gun-control-related activity before and after \SH.}
%           \label{fig:distSessionsCommon}
%\end{figure}


==> 025temporalEvolution.tex <==
%\reminder{I've updated the figures, but *not* the text/observations} 
Our second study is on the effect of the external event on the browsing behavior of the users, and for this purpose we focus on the time evolution of the browsing behaviors. %track some simple statistics over time. 

%\subsection{\nonNewsT Dataset} 
%Specifically, we compute the total number of users, sessions, total visits (we consider every unique pair <session-id, url> as one visit of the corresponding website, i.e., if one user browses the same website during different sessions, we will count each click as one visit), and new users. The time series of these statistics are presented in Fig.~\ref{fig:temporal}. 

%\begin{figure}[hb!]
%\centering
%\begin{subfigure}[b]{\columnwidth}
%      \includegraphics[width=\textwidth]{FIG/temporal_evolution_users_sessions_visits_new_users}
%        \caption{Number of total users, sessions, unique webpages, and {\it new} users per day.}
%                 \label{fig:temporal}
%  \end{subfigure}
%  
%  \begin{subfigure}[b]{\columnwidth}
%         \includegraphics[width=\textwidth]{FIG/temporal_evolution_webpages_new_content}
%          \caption{Unique webpages visited, and generation of new web content per day.}
%                   \label{fig:newContent}
%    \end{subfigure}
%    \caption{\nonNews: Temporal evolution of browsing behavior and effect of external event.}
%\end{figure}

%The first big spike in the new users time series appears the day of the event, and is followed by another spike on December 17 --3 days later--, when a petition on stricter gun control was created and signed by numerous users. Although one might expect that the number of new users would increase significantly right after the event, and then gradually decrease, the maximum number of new users appears on December 27, when many people got interested in the released Assault Weapons Ban List.
%
%Moreover, we compute the number of webpages visited, as well as the new web content generated per day. These time series are depicted in Fig.~\ref{fig:newContent}. As expected, the event on December 14 triggered the generation of significant amount of webpages, and attracted the interest of numerous users on issues related to the event, and gun control/rights. The biggest spike in the web content generation time series (as well as the second biggest spike in the new users time series) appears 3 days after the event, and is due to the creation of a petition on stricter gun control. 

\subsection{Temporal evolution of browsing activity.}
How diverse is the information browsed every day? What categories of websites do the users visit more frequently? Is the diversity affected by external events, or does it remain constant? To answer these questions, for each day, we compute the number of {\it unique URLs} in each category and present the original and normalized label distributions in Figures~\ref{fig:origDistByURLCount} and~\ref{fig:normDistByURLCount} respectively. These plots show the polarity in the webpages browsed per day. 

The gun rights websites are consistently dominant during all the days before \SH (Dec.~14), and increase after the event. In the aftermath of the shooting event, the number of gun control websites increases and becomes comparable to the gun rights webpages visited. \reviewer{I don't see the evidence of this statement in 4(a) or 4(b), in particular not the comparable numbers of control and rights sites.} Although the number of gun control websites visited drops over time, it remains higher than before the event. As far as the highly balanced and purely factual websites are concerned, a significant number of them are visited after \SH, and remain almost constant until the end of December. The first small spike in the user activity appears on December 3rd, when Bob Costas speaks out in favor of gun control during `Sunday Night Football'. 

\begin{figure}[t!]
  \centering
  \begin{subfigure}[b]{\columnwidth}
      \includegraphics[width=\textwidth]{FIG/temporal_label_distribution_url_counts}
  \caption{Original label distributions per day (unique URLs browsed per day).}
           \label{fig:origDistByURLCount}
  \end{subfigure}
  
  \begin{subfigure}[b]{\columnwidth}
          \includegraphics[width=\textwidth]{FIG/temporal_label_distribution_normalized_url_counts}
      \caption{Normalized label distributions per day (unique URLs browsed per day).}
               \label{fig:normDistByURLCount}
  \end{subfigure}
  
  \begin{subfigure}[b]{\columnwidth}
        \includegraphics[width=\textwidth]{FIG/temporal_label_distribution_visits}
    \caption{Original label distributions per day (in terms of visit frequency).}
             \label{fig:origDistByVisits}
      \end{subfigure}
    
    \begin{subfigure}[b]{\columnwidth}
        \includegraphics[width=\textwidth]{FIG/temporal_label_distribution_normalized_visits}
          \caption{Normalized label distributions per day (in terms of visit frequency).}
                   \label{fig:normDistByVisits}
        \end{subfigure}
    \caption{\nonNews / all users: Temporal evolution of user activity in terms of unique URLs (a-b) and total visits per day (c-d).} %Diversity in information browsed per day. Left: diversity by unique webpages browses. Right: diversity by visit frequency of webpages.}
\end{figure}

In addition to the unique URLs visited, we compute the daily number of {\it visits} to URLs in each category, which captures {\it how often} the users browse the available websites of each category. The original and normalized label distribution by visit frequency are presented in Figures~\ref{fig:origDistByVisits} and~\ref{fig:normDistByVisits} respectively.

%\begin{observation}
Even through the lens of number of visits, the gun rights websites are dominant both before and after \SH. 
%The purely factual and highly balanced webpages that become available after the event, attract the interest of many users, as signified by the number of visits to them. 
The spike on Dec.~17th in Fig.~\ref{fig:origDistByVisits} is due to a gun control petition (big, light blue bar) that was created and signed on that day by over 4,000 people. 
Finally, the spike on Dec.~27th corresponds to a gun control website that is visited heavily on the day of its creation, and contains information about the introduction of new legislation for banning more guns (Gun Ban List).
%\end{observation}

In Fig.~\ref{fig:normDistByVisits}, the interest lies in the sudden increase in visits to gun control (light blue) websites right after Sandy Hook, and its gradual fade and elimination one week later.

In the following analysis, we present results considering {\it all} the URLs, as well as the set of URLs after removing the Gun Ban List website -- the heavy visitation to which can affect the overall analysis.

%\begin{figure}[h!]
%  \centering
%  \begin{subfigure}[b]{\columnwidth}
%      \includegraphics[width=\textwidth]{FIG/temporal_label_distribution_visits}
%  \caption{Original label distributions per day.}
%           \label{fig:origDistByVisits}
%    \end{subfigure}
%       
%    \begin{subfigure}[b]{\columnwidth}
%    \includegraphics[width=\textwidth]{FIG/temporal_label_distribution_normalized_visits}
%      \caption{Normalized label distributions per day.}
%               \label{fig:normDistByVisits}
%    \end{subfigure}           
%    \caption{\nonNews / all users: Diversity in information browsed per day (in terms of visit frequency).}
%\end{figure}


% % % Common users % % %
%\begin{figure}[t!]
%\centering
%\begin{subfigure}[b]{0.48\textwidth}
%      \includegraphics[width=\textwidth]{FIG/temporal_evolution_users_sessions_visits_new_users-COMMON}
%        \caption{Number of total common users, sessions, unique webpages, and {\it new} users per day.}
%                 \label{fig:temporal-common}
%  \end{subfigure}
%  
%  \begin{subfigure}[b]{0.48\textwidth}
%         \includegraphics[width=\textwidth]{FIG/temporal_evolution_webpages_new_content-COMMON}
%          \caption{Unique webpages visited, and new web content accessed by the common users per day.}
%                   \label{fig:newContent-common}
%    \end{subfigure}
%    \caption{\nonNewsCommon: Temporal evolution of browsing behavior and effect of external event.}
%\end{figure}
%
%\begin{figure}[t!]
%  \centering
%  \begin{subfigure}[b]{0.48\textwidth}
%      \includegraphics[width=\textwidth]{FIG/temporal_evolution_users_sessions_visits_new_users-NEWS}
%        \caption{Number of total users, sessions, unique webpages, total visits per day. The image on the right focuses on all the days other than the day with the big spike.}
%                 \label{fig:temporalNews}
%    \end{subfigure}
%       
%    \begin{subfigure}[b]{0.48\textwidth}
%    \includegraphics[width=\textwidth]{FIG/temporal_evolution_webpages_new_content-NEWS}
%      \caption{Unique webpages visited, and generation of new web content per day.}
%               \label{fig:newContentNews}
%               \end{subfigure}           
%                   \caption{\news / all users: Diversity in information browsed per day (in terms of visit frequency).}
%\end{figure}

\subsection{Temporal evolution of browsing activity for common users.}

\begin{figure}[t!]
  \centering
  \begin{subfigure}[b]{\columnwidth}
      \includegraphics[width=\textwidth]{FIG/temporal_label_distribution_url_counts-COMMON}
  \caption{Original label distributions per day (unique URLs browsed per day).}
           \label{fig:origDistByURLCountCom}
  \end{subfigure}
  
  \begin{subfigure}[b]{\columnwidth}
          \includegraphics[width=\textwidth]{FIG/temporal_label_distribution_normalized_url_counts-COMMON}
      \caption{Normalized label distributions per day (unique URLs browsed per day).}
               \label{fig:normDistByURLCountCom}
      \end{subfigure}
  
  \begin{subfigure}[b]{\columnwidth}
        \includegraphics[width=\textwidth]{FIG/temporal_label_distribution_visits-COMMON}
    \caption{Original label distributions per day (in terms of visit frequency).}
             \label{fig:origDistByVisitsCom}
      \end{subfigure}
    
    \begin{subfigure}[b]{\columnwidth}
        \includegraphics[width=\textwidth]{FIG/temporal_label_distribution_normalized_visits-COMMON}
          \caption{Normalized label distributions per day (in terms of visit frequency).}
                   \label{fig:normDistByVisitsCom}
        \end{subfigure}
    \caption{\nonNewsCommon: Temporal evolution of user activity in terms of unique URLs (a-b) and total visits per day (c-d).}
    \label{fig:diversity_common_users}
\end{figure}

\reviewer{You don't provide any real comparison between all users and common users, only descibe the behavior of common users. If there are significant differences between all and common, some test results need to be provided.}
In this section, we want to understand how users react to the shooting event. Does the latter change the browsing behavior of the users? In order to answer this question, we focus on the {\it common} users, i.e., the users that were already interested in the topic of gun control/rights before the event, and continue browsing on-topic websites after. %We answer these questions by focusing on the set of common users, as defined in Sec.~\ref{sec:categories}.

%We start our analysis by presenting how the browsing behavior of the common users evolves over time (Fig.~\ref{fig:temporal-common} and~\ref{fig:newContent-common}).


%\begin{observation}
%\reminder{to refine...} Many users added on Dec. 3 - bob costas' commentary. Total sessions increase after the event - spikes similar to the ones observed for the overall population.
%\end{observation}
%
%%\begin{observation}
%%\reminder{to refine...} Fig.~\ref{fig:temporal-common} - Many users added on Dec. 3 - bob costas' commentary. Total sessions increase after the event - spikes similar to the ones observed for the overall population.
%%\end{observation}
%
%\begin{observation}
%\reminder{to refine...} Fig.~\ref{fig:newContent-common} - Access almost the same number of new webpages every day - small fluctuations. Most unique websites visited on Dec. 18 \reminder{why?}
%\end{observation}


As far as the diversity of the webpages visited by the common users is concerned (Figure~\ref{fig:diversity_common_users}), it seems to follow a quite different pattern from the one of the overall population. 
%
First of all, in November we observe weekly periodicity in the daily number of visits to gun control/rights pages, with the peak of activity on Wednesdays, and significantly lower activity during the weekends. This is verified by doing Discrete Fourier Transform to the time series; the component with the maximum amplitude corresponds to 7 days. Moreover, the activity is lower during the weekend than in the weekdays even after the shooting; the event happened on Friday, but the peak of interest on related topics occurred on Monday, December 17. Limited activity is also observed on the days surrounding Thanksgiving, and Christmas holidays. Finally, the periodic pattern that is observed during November, fades out in December, after Costas' commentary on Dec.~3rd, and especially after the shooting in mid December.
%\begin{observation}

As far as the diversity of information is concerned, before the event, the common users visit almost exclusively websites supporting gun rights (moderate or extreme). 
  The event has as effect the exposure of the users to some purely factual and highly balanced websites, the number of which drops as the time goes by. The only day with significant visits to moderate gun control websites is December 27, when the introduction of a new gun ban list was announced. It is worth mentioning that while in the overall population, there was increased number of visits to gun control websites on December 17th, when the gun control petition was created, there is no significant such activity among the common users. This observation, in conjunction with the periodic activity, may be signifying that the users that are active during the whole time period possess guns for hunting or other purposes, and are visiting related forums daily, or at least weekly.
%\end{observation}



% % % News Dataset % % %

%%% pnb: commenting out this section for WWW submission.  The new content 
%%%   generation measurement is interesting and we should consider doing it
%%%   conditioned on label or some other variable.

%% \subsection{\newsT Dataset} 

%% %\reminder{add new content plots}

%% We conclude the temporal analysis with some observations on the \news dataset during December. As expected, there is a dominant spike on the day of the event (Fig.~\ref{fig:temporalNews}); the total sessions, websites and visits increase abruptly on the day of the shooting.
%% %
%% %a big number of users starts following the news on the shooting event. 
%% The interest of users decreases gradually over the course of the subsequent days, as denoted by the number of visits and sessions. Some significantly smaller spikes are observed on Dec/ 3rd due to the news on Bob Costas' (NBC broadcaster) gun control commentary, and Dec.~17th because of news covering the gun control petition. 

%% \begin{figure}[h!]
%%   \centering
%%       \includegraphics[width=0.48\textwidth]{FIG/temporal_evolution_users_sessions_visits_new_users-NEWS}
%%   \caption{\news: Number of total users, sessions, unique webpages, total visits per day. The image on the right focuses on all the days before and after the event, as the spike in the users  }
%%            \label{fig:temporalNews}
%% \end{figure}

%% We also attempt to understand how new content is generated because of an external event. To this end, we use the daily visits to webpages as a proxy to estimate the newly generated content: we assume that a webpage $w$ is new on day $t$ if it has not been visited by anyone during the days $t-1$. % As far as the new web content generation is concerned (
%% The new web content generation follows the expected curve (Fig.~\ref{fig:newContentNews}). The most relevant news articles are generated on the day of the event, and gradually decrease in the subsequent days (although the generation of web content remains higher than before \SH). 

%% %\reminder{Do we want to show the time series for the news dataset, for the common users? I think that if we show something, it should be about the users that are common in the \nonNews dataset...}
%% %
%% \begin{figure}[h!]
%%   \centering
%%       \includegraphics[width=0.45\textwidth]{FIG/temporal_evolution_new_content-NEWS}
%%   \caption{\news: Unique webpages visited, and generation of new web content per day.}
%%            \label{fig:newContentNews}
%% \end{figure}

==> 030change_in_polarity.tex <==
%\reminder{Drop altogether or keep some things, given the updates in the previous section} Do external events affect the polarity in controversial topics? In this section, we answer this question by assessing the polarity on gun control before and after the \SH shooting.
%
%Let $V_i$ be the number of sessions that include a visit to website $w_i$. We consider the union set of the top-$k$ websites, ordered by $V_i$, visited before and after \SH. For each time period, we compute the (normalized) percentage of the top-$k$ websites that belong to each category. That is, for category $c_j$ we report the percentage $\sum_{w_i \in c_j \wedge i \in \{1,\dots,k\}}{V_i}/V$, where $V = \sum_{i=1}^{k}{V_i}$ is the total number of visits to websites in the union set, during the corresponding time period.
%
%Table~\ref{tab:polarityChange1} shows the relative, and absolute number of visits in each category for $k=100$ before (left) and after (right) \SH. Table~\ref{tab:polarityChange2} presents the polarity for the top-1000 ($k=1000$) websites; this is also depicted in Fig.~\ref{fig:polarityChange2}. 
%
%\begin{figure}[h!]
%  \centering
%      \includegraphics[width=0.45\textwidth]{FIG/normalized_percent_visits_top1000}
%  \caption{Effect of external event on all the users: polarity change in terms of visitation.}
%           \label{fig:polarityChange2}
%\end{figure}
%
%\begin{observation}
%The shooting event increases the polarization: it seems that the event causes mobility from balanced and moderate-gun-rights viewpoints towards less neutral stances: moderate and extreme gun control, as well as extreme gun rights.
%\end{observation}
%
%Specifically, the relative number of visits to moderate gun rights websites decreases dramatically after the shooting, while moderate gun control webpages attract attention. Moreover, the extreme gun rights webpages become more popular than the moderate ones.
%
%\begin{observation}
%The event draws the attention of more users to the gun control/rights debate, as implied by the increased number of visits to relevant websites.
%\end{observation}
%
%To quantify the change in the polarity, we also compute the {\it entropy} of the labels of the top websites. Formally, let $X$ be the category/label of a popular website during December (one of the top-k URLs before/after \SH). $X$ takes values $x_1$ = ``Highly Balanced'', $x_2$= ``Moderate Gun Control'', $x_3$ = ``Extreme Gun Control'', $x_4$ = ``Extreme Gun Rights, $x_5$ = ``Moderate Gun Rights'', and $x_6$ =	``Purely Factual'', and its probability mass function is $P(X)$. The Shannon entropy of $X$ is given by $$H(X) = E[-\ln{P(X)}] = -\sum_i{P(X=x_i)*\ln{P(X=x_i)}}.$$
%
%For the top-100 websites, the entropy increases from 1.85 to 2.33 after the event. Similarly, for the top-1000 webpages, it increases from 1.65 to 2.41 after the shooting.
% 
%\begin{observation}
%The increase of the entropy of the labels after the event signifies that the viewpoints of the users become less predictable. This is expected, as there is shift in the supported views, as well as emergence of new opinions (moderate gun control). 
%\end{observation}
%
%%In both cases, we observe that there is mobility from balanced viewpoints (``Purely Factual'' and ``Highly Balanced'') towards less neutral stances. As far as gun rights are concerned, it seems that after the shooting the users tend to support more extreme positions, as the percentage of the visited webpages in the ``Extreme Gun Rights'' category increases, while the percentage in ``Moderate Gun Rights'' decreases. Moreover, the event had as a result the appearance of ``Moderate Gun Control'' webpages in the top-10 and top-20 lists; it is worth mentioning that no website supporting gun control was among the top-10 or top-20 websites before \SH. Therefore, it seems that external events affect the positions of the users, and increase the polarization.
%
%\begin{table*}[htbp]
%  \centering
%  \caption{TOP-100 websites: normalized percent and absolute numbers of website visits in each category before and after \SH.}
%  \resizebox{\textwidth}{!}{
%    \begin{tabular}{l|rr||rr||c}
%        \toprule
%              & \multicolumn{2}{c||}{\textbf{Before \SH}} & \multicolumn{2}{c||}{\textbf{After \SH}} &  
%                            \multicolumn{1}{c}{\textbf{ \% Change}} \\
%                      \midrule
%                            & \multicolumn{1}{c}{\textbf{Normalized \% of visits}} & \multicolumn{1}{c||}{\textbf{Number of visits}} & \multicolumn{1}{c}{\textbf{Normalized \% of visits}} & \multicolumn{1}{c||}{\textbf{Number of visits}} &  \\
%            \textbf{Highly Balanced} & 22.17\% & 1,434 & 22.50\% & 11,994 & UP \\
%                \textbf{Moderate Gun Control} & 0.06\% & 4     & 18.15\% & 9,671 & UP \\
%                \textbf{Extreme Gun Control} & 1.31\% & 85    & 3.10\% & 1,653 & UP \\
%                \textbf{Extreme Gun Rights} & 21.35\% & 1,381 & 33.10\% & 17,641 & UP \\
%                \textbf{Moderate Gun Rights} & 46.98\% & 3,039 & 12.58\% & 6,703 & DOWN \\
%                \textbf{Purely Factual} & 8.13\% & 526   & 10.57\% & 5,635 & UP \\
%        \bottomrule
%        \end{tabular}%
%    }
%  \label{tab:polarityChange1}%
%\end{table*}%
%
%% Table generated by Excel2LaTeX from sheet 'Polarity Change'
%\begin{table*}[htbp]
%  \centering
%  \caption{TOP-1000 websites: normalized percent and absolute numbers of website visits in each category before and after \SH.}
%  \resizebox{\textwidth}{!}{
%    \begin{tabular}{l|rr||rr||c}
%        \toprule
%              & \multicolumn{2}{c||}{\textbf{Before \SH}} & \multicolumn{2}{c||}{\textbf{After \SH}} &  
%              \multicolumn{1}{c}{\textbf{\% Change}} \\
%        \midrule
%              & \multicolumn{1}{c}{\textbf{Normalized \% of visits}} & \multicolumn{1}{c||}{\textbf{Number of visits}} & \multicolumn{1}{c}{\textbf{Normalized \% of visits}} & \multicolumn{1}{c||}{\textbf{Number of visits}} &  \\
%        \textbf{Highly Balanced} & 12.30\% & 1,517 & 19.19\% & 13,940 & UP \\
%            \textbf{Moderate Gun Control} & 0.43\% & 53    & 15.08\% & 10,959 & UP \\
%            \textbf{Extreme Gun Control} & 0.97\% & 120   & 3.55\% & 2,578 & UP \\
%            \textbf{Extreme Gun Rights} & 23.66\% & 2,917 & 30.51\% & 22,169 & UP \\
%            \textbf{Moderate Gun Rights} & 57.14\% & 7,046 & 17.96\% & 13,045 & DOWN \\
%            \textbf{Purely Factual} & 5.50\% & 678   & 13.68\% & 9,938 & UP \\
%        \bottomrule
%        \end{tabular}%
%    }
%  \label{tab:polarityChange2}%
%\end{table*}%
%
%\paragraph{Common Users.}
%The same analysis is done for the common users, and the results for the top-100 and top-1000 websites are presented in Tables~\ref{tab:polarityChangeCommonTop100} and \ref{tab:polarityChangeCommonTop1000} respectively. The change in polarity is also depicted in Fig.~\ref{fig:polarityChange2_common}.
%
%\begin{figure}[h!]
%  \centering
%      \includegraphics[width=0.45\textwidth]{FIG/normalized_percent_visits_top1000_COMMON_users}
%  \caption{Effect of external event on common users: polarity change in terms of visitation. \reminder{Visits to the same set of URLs by the same users. If a URL did not exist before S.H., it has zero visits then.}}
%           \label{fig:polarityChange2_common}
%\end{figure}
%
%\begin{observation}
%The shooting event increases the polarization for the same set of users as well. However, it seems that the common users are members of the gun lobby, and the event causes mainly shift from moderate to extreme viewpoints about their gun rights.
%\end{observation}
%
%A small increase in moderate gun control is also observed, while the relative numbers of visits to balanced webpages remain almost constant.
%
%\begin{observation}
%After the event, the absolute numbers of visits to extreme gun rights and moderate gun control websites increase significantly (135$\times$, 2$\times$ resp.).
%\end{observation}
%
%For the top-100 websites, the entropy increases from 1.32 to 1.51 after the event. Similarly, for the top-1000 webpages, it increases from 1.19 to 1.37. As for all the users, the entropy increases after the shooting, but in this case the increase is smaller. This is in agreement with our previous observation that the common users are mainly supporters of gun rights, and the webpages they visit reflect their viewpoints both before and after the event.
%
%% Table generated by Excel2LaTeX from sheet 'Polarity Change Merged top-k(2)'
%\begin{table*}[htbp]
%  \centering
%  \caption{TOP-100 websites for the common users: normalized percent and absolute numbers of website visits in each category before and after \SH.}
%    \resizebox{\textwidth}{!}{
%    \begin{tabular}{l||rr||rr||r}
%    \toprule
%       & \multicolumn{2}{c||}{\textbf{Before \SH}} & \multicolumn{2}{c||}{\textbf{After \SH}} &  
%                    \multicolumn{1}{c}{\textbf{\% Change}} \\
%
%                    & \multicolumn{1}{c}{\textbf{Normalized \% of visits}} & \multicolumn{1}{c||}{\textbf{Number of visits}} & \multicolumn{1}{c}{\textbf{Normalized \% of visits}} & \multicolumn{1}{c||}{\textbf{Number of visits}} &  \\
%                                  \midrule
%    \textbf{Moderate Gun Control} & 0.05\% & 1     & 4.92\% & 135   & UP \\
%        \textbf{Extreme Gun Control} & 0.80\% & 17    & 0.36\% & 10    & DOWN \\
%        \textbf{Extreme Gun Rights} & 22.92\% & 485   & 33.47\% & 919   & UP \\
%        \textbf{Moderate Gun Rights} & 66.97\% & 1,417 & 55.83\% & 1,533 & DOWN \\
%        \textbf{Purely Factual} & 2.17\% & 46    & 1.46\% & 40    & DOWN \\
%    \bottomrule
%    \end{tabular}%
%    }
%  \label{tab:polarityChangeCommonTop100}%
%\end{table*}%
%
%
%% Table generated by Excel2LaTeX from sheet 'Polarity Change Merged top-k(2)'
%\begin{table*}[htbp]
%  \centering
%  \caption{TOP-1000 websites for the common users: normalized percent and absolute numbers of website visits in each category before and after \SH.}
%    \resizebox{\textwidth}{!}{
%    \begin{tabular}{l||rr||rr||r}
%    \toprule
%     & \multicolumn{2}{c||}{\textbf{Before \SH}} & \multicolumn{2}{c||}{\textbf{After \SH}} &  
%                  \multicolumn{1}{c}{\textbf{\% Change}} \\
%                  & \multicolumn{1}{c}{\textbf{Normalized \% of visits}} & \multicolumn{1}{c||}{\textbf{Number of visits}} & \multicolumn{1}{c}{\textbf{Normalized \% of visits}} & \multicolumn{1}{c||}{\textbf{Number of visits}} &  \\
%              \midrule
%    \textbf{Extreme Gun Control} & 0.30\% & 17    & 0.26\% & 20    & DOWN \\
%        \textbf{Moderate Gun Control} & 0.02\% & 1     & 1.90\% & 144   & UP \\
%        \textbf{Moderate Gun Rights} & 67.21\% & 3,843 & 56.49\% & 4,286 & DOWN \\
%        \textbf{Extreme Gun Rights} & 27.34\% & 1,563 & 36.80\% & 2,792 & UP \\
%        \textbf{Purely Factual} & 1.68\% & 96    & 1.98\% & 150   & UP \\
%    \bottomrule
%    \end{tabular}%
%    }
%  \label{tab:polarityChangeCommonTop1000}%
%\end{table*}%
%
%


==> 032communities.tex <==

%\subsection{Dynamics of the communities}

Can we find communities in the users who get informed on gun-policy related issues and track their evolution after the shootings? To achieve this, we characterize the users based on the types of websites they visit during the two time periods, and form 3 communities: gun control, gun rights, and balanced/factual. %In this section, we observe how the dynamics of these communities change (if applicable) after the shooting.

For the characterization of user $u$, we assign a score defined as:
$$ s_u = \sum_{x \in \mathcal{L}}w(x)\cdot n_{u,x},$$
where $\mathcal{L}$ is the set of labels \{gun control, gun rights, balanced/factual\}, $n_{u,x}$ is the number of domains in category $x$ that user $u$ visited, and $w(x)$ is a weight function:
$$
w(x) = \left\{
	\begin{array}{ll}
	-1 & \mbox{if $x$ = gun rights}\\
	\;\; 0 & \mbox{if $x$ = balanced}\\
	+1 & \mbox{if $x$ = gun control}
	\end{array}
\right.
$$
%$$  +1, if x = \text{gun control} $$
%$$ w(x) = 0, if x = \text{balanced/factual} $$
%$$ -1, if x = \text{gun rights}. $$

Then, the sign of the score $s_u$ defines the community to which user $u$ belongs
$$
\textit{community}(u) = \left\{
	\begin{array}{ll}
	\text{gun rights} & \mbox{if } \textit{sign}(s_u)<0\\
	\text{balanced} & \mbox{if } \textit{sign}(s_u)=0\\
	\text{gun control} & \mbox{if } \textit{sign}(s_u)>0
	\end{array}
\right.
$$

%$$ \text{gun control}, \textbf{if} sign(s_u)>0 $$
%$$community(u) = \text{balanced}, \textbf{if} sign(s_u)=0 $$
%$$\text{gun rights}, \textbf{if} sign(s_u)<0.$$

\noindent For example, if a user visited 0 gun control, 1 balanced, and 1 gun rights webpage, she is assumed to ``support'' gun rights. As before, we distinguish two cases in the analysis: before and after removing the gun ban list website.

\begin{figure}[t]
    \centering
     \includegraphics[width=0.85\columnwidth]{FIG/053communities_dynamics}
     \caption{Before removing the gun ban list website: Transitions between communities after the event.}
     \label{fig:transitions}
\end{figure}

\textbf{Before removing the gun ban list website.} Based on the definitions given above, we assign each user to a community (state) before and after \SH, and compute the transition matrix, which is given graphically in Fig.~\ref{fig:transitions}. The size of the states reflects the relative size of the communities, and the weight of the arrows is related to the probability of transitioning from one state to another after the shooting (note that the weights of the outgoing arrows from each state add up to 1). The majority of users from each category seem to be shifting to the gun rights community, an observation which naturally leads us to the next question: is there equilibrium in the ``system'' or do the communities change size after the event? The short answer is that the system exhibits almost equilibrium. Let the triplet ($p_c$, $p_b$, $p_r$) denote the probabilities of belonging to the gun control, balanced, and gun rights communities respectively. Then, before the event the probabilities are (7.79\%, 19.03\%, 73.13\%) and after the event (6.66\%, 19.55\%, 73.79\%), which shows that the communities maintain almost the same size. To be more precise, the gun control community slightly shrinks, while the other two groups increase in size by a very small percent.

\textbf{After removing the gun ban list website (outlier on Dec.~27th).} As in the previous section, we repeat the analysis after excluding the outlier webpage. The transition matrix is given in Table~\ref{tab:transitions}. The triplets of probabilities, which are described in the previous paragraph, are $(p_c, p_b, p_r)_{BEFORE} =$ (7.79\%, 20.32\%, 71.89\%) and $(p_c, p_b, p_r)_{AFTER} =$ (6.90\%, 17.55\%, 75.54\%). Hence, in this case, the gun control and balanced communities shrink, while the gun rights community attracts new members.

%How many users converted from one category to another? \reminder{Describe the characterization of the users}

%\danai{add trajectories of 2-3 users and observations from end-of-internship presentation}

\begin{table}[t]
  \centering
  \caption{After removing the gun ban list website: Transition matrix between states/communities after \SH.}
  {\scriptsize
%    \resizebox{\columnwidth}{!}{
    \begin{tabular}{c|rccc}
%    \resizebox{\textwidth}{!}{
    \toprule
    \multicolumn{2}{c}{\multirow{2}[4]{*}{}} & \multicolumn{3}{c}{\textbf{AFTER}} \\
    \midrule
    & & \textbf{Gun Control} & \textbf{Balanced} & \textbf{Gun Rights} \\
    \multirow{3}[6]{*}{\textbf{BEFORE}} & \textbf{Gun Control} & 31.65\% & 21.52\% & 46.84\% \\
          & \textbf{Balanced} & 9.71\% & 24.27\% & 66.02\% \\
          & \textbf{Gun Rights} & 3.43\% & 15.23\% & 81.34\% \\
    \bottomrule
%    }
    \end{tabular}%
    }
  \label{tab:transitions}%
  
\end{table}%


==> 041bridges.tex <==
In this section, we study nodes (webpages) that are candidates for ``bridges'', i.e., nodes that act as connectors between webpages that support opposing viewpoints.

The candidates that we investigate here are the following: 
\begin{itemize*}
\item {\bf HUBs:} webpages that are connected to numerous webpages -- i.e., webpages that have high degree, independent of the domains.
\item {\bf heterogeneous-HUBs:} webpages with neighbors from numerous different domains.
\end{itemize*}

Our goal is to understand the properties of the bridge nodes. To this end, we want to compute the entropy of the neighbors' labels in each category, and see if there is a correlation between the graph properties of the nodes, and their semantic properties (linking webpages of opposing viewpoints).

%% Table generated by Excel2LaTeX from sheet 'Outgoing_domains'
%\begin{table*}[htbp]
%  \centering
%  \caption{{\bf Outlinks} after \SH: Top-20 websites with neighbors from different domains.}
%    \begin{tabular}{lr}
%    \toprule
%    \textbf{URLs AFTER \SH} & \textbf{Outgoing domains} \\
%    \midrule
%    http://home.nra.org & 87 \\
%    http://en.wikipedia.org/wiki/second\_amendment\_to\_the\_united\_states\_constitution & 83 \\
%    http://justfacts.com/guncontrol.asp & 57 \\
%    http://feinstein.senate.gov/public/index.cfm/assault-weapons & 53 \\
%    http://pages.townhall.com/campaign/2nd-amendment & 45 \\
%    http://en.wikipedia.org/wiki/sandy\_hook\_elementary\_school\_shooting & 43 \\
%    http://en.wikipedia.org/wiki/gun\_violence\_in\_the\_united\_states & 42 \\
%    http://nra.org/home.aspx & 40 \\
%    http://en.wikipedia.org/wiki/list\_of\_countries\_by\_firearm-related\_death\_rate & 39 \\
%    http://en.wikipedia.org/wiki/gun\_laws\_in\_the\_united\_states\_(by\_state) & 35 \\
%    http://en.wikipedia.org/wiki/gun\_politics & 32 \\
%    http://en.wikipedia.org/wiki/national\_rifle\_association & 32 \\
%    http://en.wikipedia.org/wiki/concealed\_carry\_in\_the\_united\_states & 32 \\
%    http://law.cornell.edu/constitution/second\_amendment & 31 \\
%    http://usconcealedcarry.net/adcenter/?id=bing\&sid=minisiteadcenterlandingpage & 30 \\
%    http://gunowners.org & 28 \\
%    http://rense.com/general85/obs.htm & 28 \\
%    http://nraila.org & 28 \\
%    http://en.wikipedia.org/wiki/gun\_politics\_in\_the\_united\_kingdom & 28 \\
%    http://en.wikipedia.org/wiki/virginia\_tech\_massacre & 27 \\
%    \bottomrule
%    \end{tabular}%
%  \label{tab:addlabel}%
%\end{table*}%
%
%
%
%% Table generated by Excel2LaTeX from sheet 'Outgoing_domains'
%\begin{table*}[htbp]
%  \centering
%  \caption{{\bf Inlinks} after \SH: Top-20 websites with neighbors from different domains.}
%    \begin{tabular}{lr}
%    \toprule
%    \textbf{URLs AFTER \SH} & \textbf{Incoming domains} \\
%    \midrule
%    http://feinstein.senate.gov/public/index.cfm/assault-weapons & 116 \\
%    http://home.nra.org & 113 \\
%    http://en.wikipedia.org/wiki/second\_amendment\_to\_the\_united\_states\_constitution & 88 \\
%    http://pages.townhall.com/campaign/2nd-amendment & 63 \\
%    http://justfacts.com/guncontrol.asp & 54 \\
%    http://nra.org/home.aspx & 51 \\
%    http://en.wikipedia.org/wiki/sandy\_hook\_elementary\_school\_shooting & 46 \\
%    http://en.wikipedia.org/wiki/list\_of\_countries\_by\_firearm-related\_death\_rate & 43 \\
%    http://en.wikipedia.org/wiki/gun\_violence\_in\_the\_united\_states & 41 \\
%    http://gunowners.org & 40 \\
%    http://nraila.org/legislation/federal-legislation/2012/feinstein-goes-for-broke-with-new-gun-ban-bill.aspx & 37 \\
%    http://nraila.org & 34 \\
%    http://en.wikipedia.org/wiki/national\_rifle\_association & 34 \\
%    http://bradycampaign.org & 34 \\
%    http://en.wikipedia.org/wiki/gun\_laws\_in\_the\_united\_states\_(by\_state) & 33 \\
%    http://archives.gov/exhibits/charters/bill\_of\_rights\_transcript.html & 32 \\
%    http://en.wikipedia.org/wiki/gun\_politics\_in\_the\_united\_kingdom & 29 \\
%    http://usconcealedcarry.net/adcenter/?id=bing\&sid=minisiteadcenterlandingpage & 29 \\
%    http://rense.com/general85/obs.htm & 28 \\
%    http://en.wikipedia.org/wiki/gun\_politics & 28 \\
%    \bottomrule
%    \end{tabular}%
%  \label{tab:addlabel}%
%\end{table*}%

